Robotic Untangling of Herbs and Salads with Parallel Grippers

The picking of one or more objects from an unsorted pile continues to be non-trivial for robotic systems. This is especially so when the pile consists of a granular material (GM) containing individual items that tangle with one another, causing more to be picked out than desired. One of the key features of such tangle-prone GMs is the presence of protrusions extending out from the main body of items in the pile. This work characterises the role the latter play in causing mechanical entanglement and their impact on picking consistency. It reports experiments in which picking GMs with different protrusion lengths (PLs) results in up to 76% increase in picked mass variance, suggesting PL to be an informative feature in the design of picking strategies. Moreover, to counter this effect, it proposes a new spread-and-pick (SnP) approach that significantly reduces tangling, making picking more consistent. Compared to prior approaches that seek to pick from a tangle-free point in the pile, the proposed method results in a decrease in picking error (PE) of up to 51%, and shows good generalisation to previously unseen GMs.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/ext/Makefile <==
SHELL := /bin/bash
SUBDIRS := $(subst Makefile,,$(wildcard */Makefile))
CLEANDIRS = $(SUBDIRS:%=clean-%)

default: \
	tex/abbreviations.tex \
	tex/symbols.tex \
	subdirs 

clean: cleandirs

subdirs: $(SUBDIRS)

#tex/%.tex: 
#	[[ -d $@ ]] || svn export -r 46 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@
tex/abbreviations.tex: 
	[[ -d $@ ]] || svn export -r 47 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@
tex/symbols.tex:
	[[ -d $@ ]] || svn export -r 47 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@

$(SUBDIRS):
	 $(MAKE) -C $@

cleandirs: $(CLEANDIRS)
$(CLEANDIRS): 
	$(MAKE) -C $(@:clean-%=%) clean

.PHONY: subdirs $(SUBDIRS)
.PHONY: cleandirs $(CLEANDIRS)



==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/ext/tex/abbreviations.tex <==
\usepackage{xspace}
\usepackage[acronym]{glossaries}%
\glsdisablehyper % switch off hyperlinks for abbreviations

\providecommand{\newabbreviation}[2]{#1\ (\renewcommand{#1}{#2\xspace}#1)}

% months
\providecommand{\jan      }{January}
\providecommand{\feb      }{February}
\providecommand{\mar      }{March}
\providecommand{\apr      }{April}
\providecommand{\may      }{May}
\providecommand{\jun      }{June}
\providecommand{\jul      }{July}
\providecommand{\aug      }{August}
\providecommand{\sep      }{September}
\providecommand{\oct      }{October}
\providecommand{\nov      }{November}
\providecommand{\dec      }{December}

% King's
\providecommand{\KCL    }{King's College London}
\providecommand{\NMS    }{Natural and Mathematical Sciences}
\providecommand{\CORE   }{the Centre for Robotics Research}
\providecommand{\RLL    }{Robot Learning Lab}
\providecommand{\WLab   }{Wheatstone Innovation Lab}

% Universities/research institutes
\providecommand{\TUM    }{Technische Universit\"{a}t Munich}
\providecommand{\UKZN   }{University of KawaZulu Natal}
\providecommand{\MIT    }{Massachusetts Institute of Technology}

% funding bodies/schemes
\providecommand{\ERC    }{European Research Council}
\providecommand{\EPSRC  }{Engineering and Physical Sciences Research Council}
\providecommand{\CC     }{Crafts Council}
\providecommand{\JSPS   }{Japan Society for the Promotion of Science}
\providecommand{\AHDB   }{Agriculture and Horticultural Development Board}
\providecommand{\RSSB   }{Rail Safety and Standards Board}
\providecommand{\CONACYT}{Consejo Nacional de Ciencia y Tecnologia}
\providecommand{\HZOZO  }{Horizon 2020}
\providecommand{\FPZ    }{Seventh Framework Program}
\providecommand{\KTP    }{Knowledge Transfer Partnership}
\providecommand{\RIA    }{Research and Innovation Action}
\providecommand{\NIHR   }{National Institute of Health Research}
\providecommand{\DoH    }{Department of Health}
\providecommand{\GCRF   }{Global Challenges Research Fund}
\providecommand{\CTF    }{College Teaching Fund}

% other bodies
\providecommand{\IEEE   }{IEEE}

% journals, conferences
\providecommand{\TRo      }{\IEEE\ \TransactionsOn\ Robotics}
\providecommand{\TNSRE    }{\IEEE\ \TransactionsOn\ Neural \Systems\ \And\ \Rehabilitation\ \Engineering}
\providecommand{\TMech    }{\IEEE\ \TransactionsOn\ Mechatronics}
\providecommand{\IJRR     }{\International\ Journal of Robotics Research}
\providecommand{\NC       }{Neural Computation}
\providecommand{\AURO     }{Autonomous Robots}
\providecommand{\RAL      }{\IEEE\ Robotics \And\ Automation Letters}
\providecommand{\ICRA     }{\IEEE\ \International\ \ConferenceOn\ Robotics and Automation}
\providecommand{\IROS     }{\IEEE\ \International\ \ConferenceOn\ Intelligent Robots and Systems}
\providecommand{\EMBC     }{EMBS/\IEEE\ \International\ \ConferenceOf\ the \Engineering\ in Medicine \And\ Biology \Society}
\providecommand{\RSS      }{Robotics: Science and Systems}
\providecommand{\Humanoids}{\IEEE\ \International\ \ConferenceOn\ Humanoid Robots}
\providecommand{\AIM      }{ASME/\IEEE\ \International\ \ConferenceOn\ Advanced Intelligent Mechatronics}
\providecommand{\ICORR    }{\IEEE\ \International\ \ConferenceOn\ \Rehabilitation\ Robotics}
\providecommand{\BioRob   }{\IEEE\ \International\ \ConferenceOn\ Biomedical Robotics \And\ Biomechatronics}
\providecommand{\NIPS     }{Advances in Neural Information Processing Systems}
\providecommand{\ESANN    }{European Symposium on Artificial Neural Networks}

% people
\providecommand{\PI     }{principle investigator}
\providecommand{\CoI    }{co-investigator}
\providecommand{\RCoI   }{researcher co-investigator}
\providecommand{\PDRA   }{postdoctoral research assistant}
\providecommand{\UG     }{undergraduate}
\providecommand{\PG     }{postgraduate}
\providecommand{\TA     }{teaching assistant}
\providecommand{\MH     }{Matthew Howard}

% certificates/qualifications
\providecommand{\BSc}    {BSc}
\providecommand{\MSci}   {MSci}
\providecommand{\MSc}    {MSc}
\providecommand{\PhD}    {PhD}
\providecommand{\PGCAPHE}{Postgraduate Certificate in Academic Practice in Higher Education}

% machine learning
\providecommand{\RL     }{reinforcement learning}
\providecommand{\HMMs   }{hidden Markov models}

% robotics
\providecommand{\RAS    }{Robotics and autonomous systems}
\providecommand{\ROS    }{Robot Operating System}
\providecommand{\PbD    }{programming by demonstration\xspace}
\providecommand{\DoF    }{degrees of freedom\xspace}
\providecommand{\VIA    }{variable impedance actuator}
\providecommand{\EMG    }{electromyography}
\providecommand{\ECG    }{electrocardiography}
\providecommand{\EEG    }{electroencephalography}
\providecommand{\VPSA   }{variable physical stiffness actuator}
\providecommand{\CCL    }{constraint consistent learning}

% bibliographies
\providecommand{\Journal       }{Journal}
\providecommand{\JournalOf     }{Journal of}
\providecommand{\ConferenceOf  }{Conference of}
\providecommand{\ConferenceOn  }{Conference on}
\providecommand{\TransactionsOn}{Transactions on}
\providecommand{\International }{International}
\providecommand{\And           }{and}
\providecommand{\Rehabilitation}{Rehabilitation}
\providecommand{\Society       }{Society}
\providecommand{\Systems       }{Systems}
\providecommand{\Engineering   }{Engineering}

% general
\providecommand{\WP     }{work package}
\providecommand{\TRL    }{technology readiness level}
\providecommand{\SME    }{small and medium enterprise}
\providecommand{\NGO    }{non-governmental organisation}
\providecommand{\OA     }{open access}
\providecommand{\ICT    }{information and communication technology}
\providecommand{\HCI    }{human computer interfaces}





==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/ext/tex/format.tex <==
\usepackage{xspace}

% define format of some common idioms
\providecommand{\eg}{\textit{e.g.,}~} %
\providecommand{\ie}{\textit{i.e.,}~} %
\providecommand{\qv}{\textit{q.v.,}~} %
\providecommand{\apriori}{\textit{a~priori}\xspace} %
\providecommand{\etc}{\textit{etc.}} %
\providecommand{\naive}{na\"ive\xspace} %

% define page/section/figure/table/etc. referencing format
\providecommand{\figurename}{Fig.}%
\providecommand{\tablename}{Table}%
\providecommand*{\pref}[1]{p.\pageref{#1}}          % page
\providecommand*{\sref}[1]{\S\ref{s:#1}}            % section
\providecommand*{\tref}[1]{\tablename~\ref{t:#1}}   % table
\providecommand*{\fref}[1]{\figurename~\ref{f:#1}}  % figure
\providecommand*{\eref}[1]{(\ref{e:#1})}            % equation

% deal with bad hyphenation
\hyphenation{public-ations}

% inline list formatting
% use enumitem package to get inline lists, set the list format
\let\labelindent\relax %<-this prevents a conflict with IEEE \labelindent when using enumitem
\usepackage[inline]{enumitem}
\setlist{nolistsep}
\providecommand{\il}[1]{\begin{enumerate*}[label=(\roman*)]#1\end{enumerate*}}



==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/ext/tex/symbols.tex <==
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{gensymb}

% character definition
\mathchardef\mhyphen="2D   % define "math hyphen"

% equivalence relations
\providecommand{\defeq}{\vcentcolon=}

% maths
\providecommand{\R}     {\mathbb{R}}          % real numbers
\providecommand{\T}     {\top}                % transpose
\providecommand{\intd}  {\mathrm{d}}          % variable of integration
\providecommand{\bO}    {\boldsymbol{0}}      % (bold) zero
\providecommand{\bl}    {\boldsymbol{1}}      % (bold) one
\providecommand{\bnabla}{\boldsymbol{\nabla}} % (bold) derivative
\providecommand{\N}     {\mathcal{N}}         % Gaussian distribution
\providecommand{\U}     {\mathcal{U}}         % uniform distribution
\providecommand{\I}     {\mathbf{I}}          % identity matrix
\providecommand{\be}    {\mathbf{e}}          % basis vector

% functions
\providecommand{\estimated} [1]{\tilde{#1}}
\providecommand{\normalised}[1]{\hat{#1}}
\providecommand{\optimal}   [1]{\bar{#1}}
\providecommand{\pinv}      [1]{{#1}^\dagger}
\providecommand{\vectornorm}[1]{||#1||}
\providecommand{\trace}     [1]{\mathrm{Tr}[#1]}        % pseudoiverse quantity
\providecommand{\leftexp}   [2]{{\vphantom{#2}}^{#1}{#2}}

% indices
\providecommand{\nd}      {n}                              % index for data points
\providecommand{\nk}      {k}                              % index for task spaces
\providecommand{\Nd}      {\mathcal{\MakeUppercase{\nd}}}  % no. data points
\providecommand{\Nk}      {\mathcal{\MakeUppercase{\nk}}}  % no. task spaces

% inputs/outputs
\providecommand{\bx}     {\mathbf{x}}         % (bold) state
\providecommand{\nx}     {p}                  % index for elements of input/state vector
\providecommand{\dimx}   {\mathcal{\MakeUppercase{\nx}}} % input/state dimensionality
\providecommand{\by}     {\mathbf{y}}         % (bold) output/observation
\providecommand{\ny}     {r}                  % index for elements of output/observation vector
\providecommand{\dimy}   {\mathcal{\MakeUppercase{\ny}}} % output/observation dimensionality

% parameters
\providecommand{\btheta}  {\boldsymbol{\theta}}               % parameter vector
\providecommand{\ntheta}  {p}                                 % index for parameter vector elements
\providecommand{\dimtheta}{\mathcal{\MakeUppercase{\ntheta}}} % parameter dimensionality

% constrained systems
\providecommand{\bA}     {\mathbf{A}}         % constraint matrix
\providecommand{\bb}     {\mathbf{b}}         % constraint vector
\providecommand{\nb}     {s}                  % index for elements of b
\providecommand{\dimb}   {\mathcal{\MakeUppercase{\nb}}} % observation dimensionality
\providecommand{\bN}     {\mathbf{N}}         % null space projection matrix
\providecommand{\bc}     {\mathbf{c}}         % null space vector
\providecommand{\dimc}   {\dimy}              % dimensionality of null space vector
\providecommand{\bw}     {\mathbf{w}}         % image space part
\providecommand{\dimw}   {\dimy}              %
\providecommand{\bv}     {\mathbf{v}}         % null space part
\providecommand{\dimv}   {\dimy}              %

% kinematics
\providecommand{\bq}     {\mathbf{q}}         % (bold) joint angles
\providecommand{\br}     {\mathbf{r}}         % (bold) end-effector positions
\providecommand{\nr}     {q}                  % index for elements of end-effector position vector
\providecommand{\dimr}   {\mathcal{\MakeUppercase{\nr}}} %  end-effector position vector dimensionality
\providecommand{\bJ}     {\mathbf{J}}         % Jacobian
\providecommand{\qdot}   {\dot{q}}            % joint velocities
\providecommand{\bqdot}  {\dot{\bq}}          % (bold) joint velocities
\providecommand{\rdot}   {\dot{r}}            % end-effector velocities
\providecommand{\brdot}  {\dot{\br}}          % (bold) end-effector velocities
\providecommand{\ebq}    {\estimated{\bq}}    % (bold) estimated joint angles
\providecommand{\ebqdot} {\estimated{\bqdot}} % (bold) estimated joint velocities

% dynamics
\providecommand{\bF}     {\mathbf{f}}         % (bold) force
\providecommand{\qddot}  {\ddot{q}}           % joint accelerations
\providecommand{\bqddot} {\ddot{\bq}}         % (bold) joint accelerations
\providecommand{\btau}   {\boldsymbol{\tau}}  % (bold) joint torques
\providecommand{\ebqddot}{\estimated{\bqddot}}% (bold) estimated joint accelerations
\providecommand{\ebtau}  {\estimated{\btau}}  % (bold) estimated joint torques
\providecommand{\rddot}  {\ddot{r}}           % end-effector accelerations
\providecommand{\brddot} {\ddot{\br}}         % (bold) end-effector accelerations
\providecommand{\bK}     {\mathbf{K}}         % (bold) stiffness matrix
\providecommand{\bB}     {\mathbf{B}}         % (bold) damping matrix
\providecommand{\brO}    {\br_{0}}            % (bold) equilibrium position in Cartesian space

% control
\providecommand  {\bu}  {\mathbf{u}}          % (bold) commands
\providecommand  {\nu}  {q}                   % index for elements of u
\providecommand  {\dimu}{\mathcal{\MakeUppercase{\nu}}} % action dimensionality
\providecommand  {\bpi} {\boldsymbol{\pi}}    % (bold) control policy
\providecommand  {\bxdot}{\dot{\bx}}          % (bold) state velocities

% learnt models
\providecommand{\bm}     {\mathbf{m}}         % (bold) RBF or local model centres
\providecommand{\bxn}    {\bx_{\nd}}          % nth input data point
\providecommand{\byn}    {\by_{\nd}}          % nth output data point
\providecommand{\bX}     {\mathbf{X}}         % input data matrix
\providecommand{\bY}     {\mathbf{Y}}         % output data matrix

% regression/classification

% reinforcement learning

% generic symbols

% equations

% other




==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/tex/abbreviations.tex <==
% include global abbreviations
\input{ext/tex/abbreviations}

% months

% King's

% Universities/research institutes

% funding bodies/schemes

% projects

% journals, conferences

% people

% certificates/qualifications

% machine learning

% robotics
\renewcommand  {\DoF}{degree of freedom\xspace}
\providecommand{\GI} {graspability index\xspace}
\providecommand{\SP}{Spread-and-Pick\xspace}
\providecommand{\FP}{Fixed-Point-Picking\xspace}
\providecommand{\rmse}{RMSE\xspace}

% bibliographies

% general
\newacronym{CNN}{CNN}{convolution neural network}\providecommand{\CNN}{\gls{CNN}\xspace}

\newacronym{MAE}{MAE}{Mean Absolute Error}\providecommand{\MAE}{\gls{MAE}\xspace}

\newglossaryentry{GM} % long form, to enable plurals
{
	name={GM},
	description={granular material},
	first={\glsentrydesc{GM} (\glsentrytext{GM})},
	plural={GMs},
	descriptionplural={granular materials},
	firstplural={\glsentrydescplural{GM} (\glsentryplural{GM})}
}\providecommand{\GM}{\gls{GM}\xspace}\providecommand{\GMs}{\glspl{GM}\xspace}
\newacronym{SnP}{SnP}{spread-and-pick}\renewcommand{\SP}{\gls{SnP}\xspace}
\newacronym{DoF}{DoF}{degree of freedom}\renewcommand{\DoF}{\gls{DoF}\xspace}
\newacronym{FP}{FP}{fixed-point-picking}\renewcommand{\FP}{\gls{FP}\xspace}
\newacronym{GI}{GI}{graspability index}\renewcommand{\GI}{\gls{GI}\xspace}
\newglossaryentry{PL} % long form, to enable plurals
{
	name={PL},
	description={protrusion length},
	first={\glsentrydesc{PL} (\glsentrytext{PL})},
	plural={\glsentrytext{PL}s},
	descriptionplural={\glsentrydesc{PL}s},
	firstplural={\glsentrydescplural{PL} (\glsentryplural{PL})}
}\providecommand{\PL}{\gls{PL}\xspace}\providecommand{\PLs}{\glspl{PL}\xspace}


==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/tex/comments.tex <==
\usepackage{ifdraft}
% define simple todo command
\usepackage[normalem]{ulem}                                        % <- for striking text out
\usepackage{marginnote}
\setlength{\marginparwidth}{1.5cm}
\usepackage[textwidth=\marginparwidth,colorinlistoftodos]{todonotes}
\providecommand{\tinytodo}[2][]
{\todo[caption={#2}, size=\small, #1]{\renewcommand{\baselinestretch}{0.5}\selectfont#2\par}}
\providecommand{\usage}{\input{tex/usage}}
% define colours for to-dos
\colorlet{jb}{red}
\colorlet{mh}{red}
\colorlet{pr}{green}

\providecommand  {\note}[1]{{\color{gray}#1}}
\providecommand  {\done}[1]{\sout{#1}}
\providecommand  {\mhsout}{\bgroup\markoverwith{\textcolor{mh}{\rule[0.5ex]{2pt}{0.4pt}}}\ULon} % define coloured strike out
\providecommand  {\edit}[3]{\mhsout{#1}\textcolor{#3}{#2}}
\providecommand  {\jb}  [1]{\tinytodo[color=white,nolist,linecolor=jb,bordercolor=white,noinline]{\protect{\scriptsize\color{jb}#1}}}
\providecommand  {\mh}  [1]{\tinytodo[color=white,linecolor=mh,bordercolor=white,noinline]{\protect{\scriptsize\color{mh}#1}}}
\providecommand  {\pr}  [1]{\tinytodo[color=white,linecolor=pr,bordercolor=white,noinline]{\protect{\scriptsize\color{pr}#1}}}
% comment above, and uncomment below to remove todo list.
%\usepackage[disable]{todonotes}\reprovidecommand{\usage}{}%\providecommand{\mh}[3]{#3}{}{}\providecommand{\maybedo}[1]{}

%\usepackage{soul}
%\DeclareRobustCommand{\mhhl}[1]{{\sethlcolor{mh!50}\hl{#1}}}

\providecommand{\atMH} {{\color{mh}@MH}}
\providecommand{\atmh} {{\color{mh}@MH}}
\providecommand{\atPR} {{\color{pr}@PR}}

\providecommand{\commentcolourcode}{Comments colour code: 
{\color{mh}MH}, 
{\color{pr}PR}} 




==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/tex/format.tex <==
\input{ext/tex/format}
\usepackage{siunitx}

% define format of some common idioms
\providecommand{\ca}{\textit{ca.}~}   %

% define page/section/figure/table/etc. referencing format
\renewcommand{\tref}[1]{Table~\ref{t:#1}}   % table

% inline list formatting
% use enumitem package to get inline lists, set the list format
\providecommand{\cl}[1]{\begin{enumerate*}[label=(\alph*)]#1\end{enumerate*}}

% define format of numbers
\providecommand{\thousand}{k} %
\providecommand{\million} {m} %
\providecommand{\billion}{bn} %

% deal with bad hyphenation
\hyphenation{public-ations}



==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/tex/preamble.tex <==
\IEEEoverridecommandlockouts                              % This command is only needed if 
%\overrideIEEEmargins            
% Needed to meet printer requirements.

\usepackage{times}
\usepackage{graphicx}\graphicspath{{img/}{images/}}
\usepackage{epstopdf}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{multirow} 
\usepackage{multicol}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{mdwtab}
\usepackage{rotating}
\usepackage[list=off]{caption}
\usepackage{amssymb}
\usepackage{verbatim}
\usepackage{overpic}
\usepackage{amsmath}
\usepackage{subcaption}
\usepackage[utf8]{inputenc}
\usepackage[export]{adjustbox}
\usepackage[hidelinks]{hyperref}
\usepackage[normalem]{ulem}
\usepackage[background = white, text=black , arrow = black, line width=5mm]{callouts}

% set up manual labelling
\makeatletter\newcommand{\manuallabel}[2]{\def\@currentlabel{#2}\label{#1}}\makeatother

\usepackage[
backend=bibtex,
style=ieee,
url=false,
doi=false,
isbn=false,
doi=true,
eprint=false,
mincitenames=1,% specify maximum number of names to be cited in text
maxcitenames=2% specify maximum number of names to be cited in text
]{biblatex}
\addbibresource{abbreviations.bib}
\addbibresource{bibliography.bib}
\renewcommand*{\bibfont}{\footnotesize}% set fontsize to match that of ieeeconf

\input{tex/abbreviations}
\input{tex/symbols}
\input{tex/format}
\input{tex/comments}


==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/tex/symbols.tex <==
% include global symbols
\input{ext/tex/symbols}

\usepackage{siunitx} % for formatting units

% equivalence relations

% maths
\providecommand{\conv}{*} % convolution
%\providecommand{\conv}{*}          %

% functions

% indices

% inputs/outputs

% parameters

% regression/classification

% reinforcement learning

% generic symbols

% equations

% other

% graspability index
%\providecommand{\bR}     {\mathbf{R}}         % collision-free orientation
%\providecommand{\bt}     {\mathbf{t}}         % collision-free position


\providecommand{\mt}     {m_t}                  % target weight

\providecommand{\r}      {r}                  % 
\renewcommand  {\r}      {r}                  % 
\providecommand{\br}     {\mathbf{\r}}        % 
\providecommand{\rx}     {\r_x}               % x-coordinate of collision-free point
\providecommand{\ry}     {\r_y}               % y-coordinate of collision-free point
\providecommand{\rz}     {\r_z}               % collision-free insertion depth
\providecommand{\rt}     {\r_{\theta}}  % gripper orientation


\providecommand{\Or}     {\mathbf{u}} % optimal collision-free point
\providecommand{\Er}     {\mathbf{v}} % peak entanglement point
\providecommand{\Oc}     {\mathbf{O_c}}         % object contact
\providecommand{\Ocp}     {\mathbf{O_{c'}}}          % object contact

\providecommand{\gc}     {\mathbf{G_c}}   % gripper contact  
\providecommand{\gcp}     {\mathbf{G_{c'}}}   % gripper contact  


\providecommand{\wc}     {\mathbf{W_c}}   % gripper-object contact  
\providecommand{\wcp}     {\mathbf{W_{c'}}}   %gripper-object collision  

\providecommand{\g}       {\mathbf{g}}  % Gaussian
\providecommand{\G}       {\mathbf{G}} % graspability map
\providecommand{\w}       {w} % gripper width
\providecommand{\p}       {p} % pile weight
\providecommand{\l}       {l} % length of transverse ends
\providecommand{\d}       {d} % width of transverse ends 
\providecommand{\DoE}     {\vartriangle}
\providecommand{\pickpar}   {\delta}

\providecommand{\e}       {PE} % picking error
\providecommand{\m}       {m} % picked weight
\providecommand{\Q}       {q} % picked weight to pick parameter
\providecommand{\f}       {f} % picked weight to pick parameter
\providecommand{\N}       {N} % number of trials

\providecommand{\bPickpar}{\boldsymbol{\Delta}}
\providecommand{\bM}      {\mathbf{M}}
\providecommand{\D}       {\mathcal{D}}
\providecommand{\VarM}    {\Sigma_\bM}

==> Robotic Untangling of Herbs and Salads with Parallel Grippers V2/tex/usage.tex <==
\section*{Usage notes}~\\%[1ex]
\noindent Use \texttt{\textbackslash yourinitials\{your comment\}} to add comments/to dos. For example,
\underline{J}oe \underline{B}loggs adds comments using \texttt{\textbackslash jb\{Comment.\}}.\jb{These comments will appear as margin notes. They will also appear in the todo list on the first page.} \\[2ex]
\noindent Optionally, use \texttt{\textbackslash atInitials} to address your comment to someone (\eg \texttt{\textbackslash jb\{\textbackslash atMH: Please fix this.\}}).\\[2ex]
You can mark a comment as resolved using \texttt{\textbackslash done\{Comment text.\}}, (\eg \texttt{\textbackslash jb\{\textbackslash done\{\textbackslash atMH: Please fix this.\}\}}). It will then be formatted like this: \done{\atMH: Please fix this.}.\\[2ex]
\commentcolourcode\\[1ex]
\listoftodos~\\[2ex]
\clearpage\setcounter{page}{1}


==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> ext/Makefile <==
SHELL := /bin/bash
SUBDIRS := $(subst Makefile,,$(wildcard */Makefile))
CLEANDIRS = $(SUBDIRS:%=clean-%)

default: \
	tex/abbreviations.tex \
	tex/symbols.tex \
	subdirs 

clean: cleandirs

subdirs: $(SUBDIRS)

#tex/%.tex: 
#	[[ -d $@ ]] || svn export -r 46 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@
tex/abbreviations.tex: 
	[[ -d $@ ]] || svn export -r 47 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@
tex/symbols.tex:
	[[ -d $@ ]] || svn export -r 47 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@

$(SUBDIRS):
	 $(MAKE) -C $@

cleandirs: $(CLEANDIRS)
$(CLEANDIRS): 
	$(MAKE) -C $(@:clean-%=%) clean

.PHONY: subdirs $(SUBDIRS)
.PHONY: cleandirs $(CLEANDIRS)


